Principal Inertia Components and Applications

We explore properties and applications of the Principal Inertia Components (PICs) between two discrete random variables $X$ and $Y$. The PICs lie in the intersection of information and estimation theory, and provide a fine-grained decomposition of the dependence between $X$ and $Y$. Moreover, the PICs describe which functions of $X$ can or cannot be reliably inferred (in terms of MMSE) given an observation of $Y$. We demonstrate that the PICs play an important role in information theory, and they can be used to characterize information-theoretic limits of certain estimation problems. In privacy settings, we prove that the PICs are related to fundamental limits of perfect privacy.

==> backup.tex <==

\section{Backup Text}


This section has four main contributions, listed below. Some of the results presented in the section appeared in \cite{calmon_bounds_2013}.


\begin{enumerate}
\item We present an overview of the PICs and their different interpretations, summarized in Theorem \ref{thm:PIC_Charac}. 

\item We analyze properties of a measure of information (correlation) between $X$ and $Y$ based on the PICs of the joint distribution of $X$ and $Y$. The estimation of the PICs is widely studied in the field of correspondence analysis, and is used in practice to analyze categorical data.  The metric we propose, called \textit{$k$-correlation}, is defined as the sum of the $k$ largest PICs, which, in turn, are the singular values of a particular decomposition of the joint distribution matrix of $X$ and $Y$. We show that $k$-correlation generalizes both the maximal correlation and the $\chi^2$ measures of correlation.  We also prove that $k$-correlation satisfies two key properties for information measures: (i) the Data Processing Inequality and (ii) convexity in the conditional probabilities $\pygx$. 

\item We  derive a family of lower bounds for the   error probability of estimating $X$ given $Y$ based on the PICs of $\pxy$ and the marginal distribution of $X$ in Theorems \ref{thm:Bound} and \ref{thm:AdvPeM}. By applying the techniques derived in Chapter \ref{chap:InformationEstimation}, we then extend these bounds for the probability of correctly estimating a function of the hidden variable $X$ given an observation of $Y$.

\item We characterize the PICs for a wide range of distributions, namely when $X$ is a sequence of $n$ i.i.d. random variables and $Y$ is a symmetric function of $X$, presented in Theorem \ref{thm:symm}. This result is also extended to exchangeable random variables in Theorem \ref{thm:exchangeable}. 
\end{enumerate}

The PICs generalize other measures that are used in information
 theory. In particular, $\lambda_1 = \rho_m(X;Y)^2$, where $\rho_m(X;Y)$ is the
 \textit{maximal correlation} between $X$ and $Y$, defined as \cite{renyi_measures_1959}
\begin{align}
\label{eq:maxcorrdef}
  \rho_m(X;Y) &\defined \max_{\substack{\EE{f(X)}=\EE{g(Y)}=0\\ \EE{f(X)^2}=\EE{g(Y)^2}=1}}\ExpVal{}{f(X)g(Y)}.
\end{align}
% 
In Section \ref{sec:charac}, we discuss how to compute the PICs and provide  alternative characterizations.  Compared to mutual information, the PICs  provide a finer-grained decomposition of the correlation between $X$ and $Y$.

We propose a  metric of information called $k$-correlation, defined as
 $ \calJ_k(X;Y) \defined \sum_{i=1}^k \lambda_i(X;Y)$.
This metric satisfies two key
properties:

\begin{itemize}
  \item Convexity in $\pygx$ (Theorem \ref{thm:convex});
  \item Data Processing Inequality (Theorem \ref{lem:dataProc}). This is also satisfied by
      $\lambda_1(X;Y),\dots,\lambda_d(X;Y)$ individually,
    \end{itemize}
and, consequently, is an information measure as per Def. \ref{defn:informationMeasure}.

By making use of the fact that the principal inertia components satisfy the Data Processing Inequality, we are able to derive a family of bounds for $P_e(X|Y)$ in terms of $\px$ and $\lambda_1(X:Y),\dots,\lambda_d(X;Y)$, described in Theorem \ref{thm:Bound}. This result sheds light on the relationship of $P_e(X|Y)$ with   the principal inertia components.

One immediate consequence of Theorem \ref{thm:Bound} is a useful scaling law for $P_e(X|Y)$ in terms of the largest principal inertia (i.e. maximal correlation). Let $X=1$ be the most likely outcome for $X$. Corollary \ref{cor:coolBounds} proves that the advantage an adversary has of guessing $X$, over the trivial solution of simply guessing the most likely outcome of $X$ (say $X=1$), satisfies
% \begin{equation} 
%   \Adv(X|Y) \defined \left|1-\px(1)-P_e(X|Y)\right|\leq O\left(\sqrt{\lambda_1(X;Y)}\right).
% \label{eq:advGuess}
% \end{equation}



\section{Main Contributions of PIC-IT}

This chapter presents different applications of the PICs to information theory, and is based on the author's work in \cite{calmon2014exploration}. In Section \ref{sec:functions}, we demonstrate that the PICs have a role in channel transformations very similar to that of filter coefficients in a linear filter. Here,  functions of a hidden variable are analogous to the input signals of the filter. This is illustrated through an example in binary additive noise channels, where we argue that the binary symmetric channel is somewhat equivalent to a ``low-pass filter''. We then use this interpretation to study the ``one-bit function conjecture'' \cite{kumar_which_2013}. We  present further evidence for that conjecture here, and introduce another, related conjecture based on the discussion.

The new conjecture (cf. Conjecture \ref{conj}), albeit not proved, is more general than the ``one-bit function conjecture''. It states that, given a symmetric distribution $\pxy$, if we generate a new distribution $q_{X,Y}$ by making all the PICs of $\pxy$ equal to the largest one, then the new distribution is ``more informative'' about bits of $X$. By ``more informative'', we mean that, for any 1-bit function $b$, $I(b(X);Y)$ is larger under $q_{X,Y}$ than  under $\pxy$. Indeed, from the previous discussion and from an estimation-theoretic perspective, any function of $X$ can be estimated with smaller MMSE when considering $q_{X,Y}$ than $\pxy$. Furthermore, in this case, we show that $q_{X,Y}$ is a $q$-ary symmetric channel. This conjecture, if proven, would imply as a corollary the original one-bit function conjecture.

We resolve the one-bit function conjecture in a specific setting in Section \ref{sec:estimators}. Instead of considering the mutual information between $b(X)$ and $Y$, we study the mutual information between $b(X)$ and a one-bit estimator $\hat{b}(Y)$. We show in Theorem \ref{thm:Estimators} that, when $\hat{b}(Y)$ is an unbiased estimator, the information that $\hat{b}(Y)$ carries about $b(X)$ can be upper-bounded for a wide range of information measures. This result also leads to bounds on estimation error probability that recovers a particular form of the result stated in Theorem \ref{thm:Bound}.

